SciCo: Hierarchical Cross-Document Coreference for Scientific Concepts

Determining coreference of concept mentions across multiple documents is a fundamental task in natural language understanding. Previous work on cross-document coreference resolution (CDCR) typically considers mentions of events in the news, which seldom involve abstract technical concepts that are prevalent in science and technology. These complex concepts take diverse or ambiguous forms and have many hierarchical levels of granularity (e.g., tasks and subtasks), posing challenges for CDCR. We present a new task of Hierarchical CDCR (H-CDCR) with the goal of jointly inferring coreference clusters and hierarchy between them. We create SciCo, an expert-annotated dataset for H-CDCR in scientific papers, 3X larger than the prominent ECB+ resource. We study strong baseline models that we customize for H-CDCR, and highlight challenges for future work.

==> sections/ethics.tex <==
\section{Ethics Statement}

Our choice to focus on computer science papers was motivated by the prevalence of methods and tasks in these papers are a rich examples for our H-CDCR problem setting, and the authors' expertise in this area.  Further experiments on other scientific domains are necessary in order to ensure broad applicability of the techniques.  Likewise, our choice to focus on English documents was for similar reasons and comes with the same caveat.  We focus on open-access papers in this work in order to ensure our data set can be released in full.  Annotators for the experiments in this paper were paid an average of USD\$XXX/hour.

==> tables/coref_hard_test.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}{lll}
%     \toprule
%          Test subset & Unified & Edit dist. \\
%          \midrule
%         Full & 78.8 & 55.4 \\
%         Lowest 10\% (edit dist.)  & 67.2 & 34.7 \\
%         Lowest 20\% (edit dist.)  & 73.2 & 38.8 \\
%         Curated (lexically diverse) & 68.7 & 40.4 \\
%         \bottomrule
%     \end{tabular}
%     \caption{\tom{we need to either (1) make this more prominent (2) remove coref conll from the main table, move here} CoNLL F1 results of the Unified model and edit-distance baseline on the entire test set, the 10\% and 20\% lowest scoring topics when ranked by performance using an edit-distance baseline, as well as the examples obtained with the curated list of lexically diverse candidates (§\ref{subsubsec:resources})}.
%     \label{tab:coref_analysis_results_test_set}
% \end{table}

==> tables/iaa.tex <==
% \begin{table}[]
%     \centering
%     \resizebox{0.48\textwidth}{!}{
%     \begin{tabular}{llll}
%         \toprule
%          Evaluation metric & Average & Max \\
%          \midrule
%          Coreference CoNLL F1 & 82.7 (±2.5) & 85.8  \\
%         %  Coreference MUC &  89.6 (±1.9) \\
%          AUC Multiclass & 85.3 (±2.7) & 89.8 \\
%          Connected Components CoNLL F1 & 82.6 (±2.1) & 85.6 \\
%          Hierarchical relations F1 & 63.0  (±2.4) & 66.9 \\
%         %  Shortest path - directed TN & 87.8 (±1.0) \\
%          Shortest Path Ratio & 64.5 (±3.5) & 70.0 \\
%         %  Shortest path - undirected TN & 75.8 (±1.5) \\
%         %  Shortest path - undirected  & 66.6 (±2.5) \\
%         \bottomrule
%     \end{tabular}}
%     \caption{Average and maximum Inter Annotator Agreement on 40 topics with the relevant evaluation metrics. Agreement scores are computed on the micro-average F1 scores of all pairs of annotators, considering one as gold, and the other as system. \tom{add macro}}
%     \label{tab:iaa}
% \end{table}


\begin{table}[!t]
    \centering
    \resizebox{1\columnwidth}{!}{
    \begin{tabular}{llll}
        \toprule
          Metric & Avg & Max(micro) & Max(macro) \\
         \midrule
         Coref. CoNLL F1 & 82.7 (±2.5) & 85.8 & 90.2  \\
        %  Coreference MUC &  89.6 (±1.9) \\
         Cluster-Hierarchy F1 & 68.9 (±2.2) & 72.1 & 82.3 \\
         %Cluster-Hierarchy F1-50\% & 62.8 (±2.4) & 67.5 & 77.7 \\ 
         Path Distance & 64.5 (±3.5) & 70.0 & 78.4 \\
        \bottomrule
    \end{tabular}}
    \caption{\textbf{Inter-annotator Agreement}. We measure micro-averaged pairwise agreement on 40 topics (groups of candidates), considering one annotation as gold, and the other as predicted. We also report the average maximal pairwise agreement, as an ``upper bound'' measure of human performance. Max(macro) denotes an average of topic-wise maximal scores.}
    \label{tab:iaa}
\end{table}


% coref_muc        90.0  1.7
% coref_bcub       86.7  1.7
% coref_ceafe      80.6  2.1
% coref_lea        79.8  2.7
% coref_conll      85.7  1.8
% connected_muc    95.1  0.9
% connected_bcub   87.1  1.0
% connected_ceafe  68.7  3.7
% connected_lea    83.4  1.4
% connected_conll  83.6  1.7
% hypernym         58.3  3.5
% directed         64.6  3.5
% directed_tn      88.1  1.0
% undirected       66.1  2.2
% undirected_tn    76.3  1.4

==> tables/results_ablations.tex <==
\begin{table}
\begin{subtable}[c]{0.45\textwidth}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllll}
    % \begin{table}[]
    % \centering
    % \resizebox{\columnwidth}{!}{
    \toprule
    % & Coreference & \multicolumn{3}{l}{Hierarchy} & CC & Shortest Path Ratio & AUC \\
    % & CoNLL F1 & Recall & Precision & F1 & CoNLL F1 \\
    & \bf{Coreference} & \multicolumn{3}{l}{\bf{Hierarchy}} && \bf{Path} \\
    & CoNLL F1 & F1 & F1-50\% &&& Ratio \\
    % \midrule
    %     IAA &  82.7 (±2.5) & - & - & 63.0 (±2.4) &  64.5 (±3.5) & 85.3 (±2.7) \\
    \midrule
         CA\textsubscript{News} &  52.4 & 37.1 & 13.0 &&& 24.1 \\
         CA\textsubscript{Sci-News} &  43.5 & 29.2 & 12.3 &&& 21.6 \\
             \midrule
         CA\textsubscript{\data{}} & 55.2 & 23.7 & 15.8 &&& 21.2 \\
         CA\textsubscript{\data{}} + CS-RoBERTa & 57.4 & 23.5 & 16.1 &&& 23.6 \\
         CA\textsubscript{\data{}} + SciBERT & 66.8 & 23.8 & 17.8  &&& 28.4 \\
             \midrule
        %   Pipeline & \bf{77.0} & 38.8 & 29.1 &&& 43.7 \\
        %  Unified\textsubscript{LF-sentence} & 77.0 & 43.0 & 33.9 &&& 45.7 \\
          Unified\textsubscript{Longformer} & \bf{77.2} & 44.5 & \textbf{36.1} &&& \bf{47.2} \\
           Unified\textsubscript{CDLM} & 77.0 & \bf{44.8} & 35.5 &&& 45.9 \\
    \bottomrule
    \end{tabular}}
\subcaption{\textbf{Model results}. We evaluate strong CDCR baselines, and a unified multiclass model for H-CDCR that outperforms the baselines.}
\end{subtable}
\begin{subtable}[c]{\textwidth}
\centering
\end{subtable}
\begin{subtable}[c]{0.45\textwidth}
\centering
\resizebox{\columnwidth}{!}{
    \begin{tabular}{lllll}
    \toprule
    
    & \bf{Coreference} & \multicolumn{2}{l}{\bf{Hierarchy}} & \bf{Path} \\
    & CoNLL F1 & F1 & F1-50\% & Ratio \\
    \midrule
    
    $-$ unified & 77.1 ($-$0.1) & 41.6 ($-$2.9) & 32.3 ($-$3.8) & 44.2 ($-$3.0)\\
    $-$ context & 77.0 ($-$0.2) & 43.0 ($-$1.5) & 33.9 ($-$2.2) & 45.7 ($-$1.5) \\
    \bottomrule
    \end{tabular}}
\subcaption{\textbf{Ablation results}. Parentheses show the relative drop in performance. Both large context and the unified approach contribute to the scores.}
\end{subtable}
\caption{two tables side by side}
\end{table}


% \begin{table}
%     \begin{subtable}
%     \begin{tabular}{c|c}
%       a  & a \\
%      a    & a
%     \end{tabular}
%     \subcaption{}
%     \end{subtable}
    
%     \begin{subtable}
%     \begin{tabular}{c|c}
%         a & a \\
%       a  & a
%     \end{tabular}
    
%     \subcaption{}
%     \end{subtable}
    
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table}

==> tables/scico_start_per_source_type.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{llll}
    \toprule
    & Pwc & Hypernym & Curated \\
    \midrule
    Agreement & 26 & 11 & 3 \\
    Total & 374 & 99 & 58   \\
    \bottomrule
    \end{tabular}
    \caption{Distribution of the topics according to sources of distant supervision.}
    \label{tab:my_label}
\end{table}

==> tables/undirected.tex <==
\begin{table}[]
    \centering
     \resizebox{0.4\textwidth}{!}{
    \begin{tabular}{lll}
    \toprule
    Model & \phantom{aaaaaa} & Micro-Average \\
    \midrule
       IAA  &&  66.1 (±2.2)\\
        News &&  36.6 \\
        Sci-News && 32.9 \\
        \data{}\textsubscript{RoBERTa} \\
         \data{}\textsubscript{CS-RoBERTa} \\
         \data{}\textsubscript{SciBERT} \\
         Pipeline \\
         Unified && 37.2 \\
        \bottomrule
    \end{tabular}}
    \caption{Results of Shortest Path ratio using undirected graphs.}
    \label{tab:my_label}
\end{table}
